Towards Provable Secure Neighbor Discovery in Wireless Networks

In wireless systems, neighbor discovery (ND) is a fundamental building block: determining which devices are within direct radio communication is an enabler for networking protocols and a wide range of applications. To thwart abuse of ND and the resultant compromise of the dependent functionality of wireless systems, numerous works proposed solutions to secure ND. Nonetheless, until very recently, there has been no formal analysis of secure ND protocols. We close this gap in \cite{asiaccs08}, but we concentrate primarily on the derivation of an impossibility result for a class of protocols. In this paper, we focus on reasoning about specific protocols. First, we contribute a number of extensions and refinements on the framework of [24]. As we are particularly concerned with the practicality of provably secure ND protocols, we investigate availability and redefine accordingly the ND specification, and also consider composability of ND with other protocols. Then, we propose and analyze two secure ND protocols: We revisit one of the protocols analyzed in [24], and introduce and prove correct a more elaborate challenge-response protocol.

==> conclusion.tex <==
\section{Conclusions}

In this paper, we investigate how to analyze and design provably secure ND protocols, building on top of the framework introduced in~\cite{asiaccs08}. We contribute a number of extensions that enable us to model and reason about more elaborate ND protocols (CR-protocols) than those previously considered (B-protocols). Basically, our revised framework (i) models additional practical aspects of wireless communications, (ii) caters to the co-existence and interoperability of secure ND protocols with other wireless security protocols, and (iii) focuses more than our work in~\cite{asiaccs08} on sought properties that are of practical relevance, in particular, pertaining to the ND protocol availability.

%Among other findings, our analysis demonstrates the difference between
%time-based (T-) ND protocols and time-and-location-based (TL-) ND protocols. TL-protocols are correct (secure) under a practically arbitrary but computationally bounded adversary model. In that sense, they are superior to T-protocols, which secure ND against an adversary with limited relaying capabilities. In contrast, T-protocols are superior to TL-protocols in terms of availability, as the latter require line-of-sight communication.

We see this work as a step towards provably secure neighbor discovery. We outline a number of possible extensions to our framework, and open problems in the Discussion section. Among those, the seemingly most interesting one is to reason on secure ND protocols in the presence of internal adversaries.  The nature of protocols that could deal with this type of adversarial behavior, as well as some recently discovered attacks~\cite{clulow06sonear}, mandate, in our opinion, a shift from message-oriented to models that explicitly consider symbols at the physical communication layer.

%% it is not clear why only for the internal adversary the shift to symobol oriented model
%% is needed. Symbol oriented is not clear either - I would elaborate this last sentence, with a line
%% or two

%In this paper, we are concerned with the problem of secure neighbor discovery
%in wireless networks. In particular, we investigate how to analyze and design
%provably secure ND protocols. The significant number of proposals in the
%literature, reflects the importance of safeguarding ND as fundamental building
%block of wireless systems. Nonetheless, it was recently shown that it is
%impossible for a broad class of protocols to solve the problem, and that a new
%type of protocols can indeed be proven to secure ND \cite{asiaccs08}. Building
%on this work, we venture further into designing and proving correct secure ND
%protocols. To achieve this, and at the same time enable reasoning on
%correctness for practical protocols, we propose a new ND specification, and a
%new mathematical model for wireless network, participating entities,
%adversaries, and protocols.
%
%In other words, the contributions of this paper are the analysis of four secure
%ND protocols, which we prove correct, and the new elements brought in by our
%model. Our effort is novel in that it enables the formal specification of
%actual secure ND protocols. Moreover, our specification of ND, that is, the
%sought properties for any candidate protocol, considers availability as part of
%the protocol correctness. This implies that any protocol that satisfies this
%revised specification is practical, in the sense it functions reliably.
%Furthermore, we identify, and integrate in our reasoning features of wireless
%media, such as non-line-of-sight communication, that were not previously
%considered.
%
%The outcome of this paper sets the ground on provably secure ND, with the four
%analyzed protocols including two protocols in the literature and two new own
%proposals. This comparative analysis does not only move towards concrete
%protocols but also provides a comparison of their properties with respect to
%their system requirements and the capabilities of the adversary. Furthermore,
%we identify open problems: reasoning on secure neighbor discovery considering
%(i) the involvement of internal adversaries, and (ii) communication that the
%adversary can affect at the physical layer symbol level. As part of future
%work, we will introduce the necessary new elements in our model, and enable
%reasoning on types of protocols and types of adversaries that have not yet been
%considered towards correctness proofs.


==> discussion.tex <==
\section{Discussion}\label{sec:discussion}

We introduced a number of abstractions in our framework, simplifying wireless communications, for the sake of modeling and reasoning on secure ND (Sec.~\ref{sec:abstractions}). In Sec.\ref{sec:comparison}, we outline here differences between protocols in terms of requirements and satisfied properties, and sketch open problems in Sec.~\ref{sec:openproblems}.

\subsection{Abstractions and Simplifications}\label{sec:abstractions}

\textbf{Mobility and NLOS Delay.}
We assume nodes are static and NLOS delay constant over time. Otherwise, propagation delay would vary during the transmission of a message. In some cases, mobility and NLOS delay changes are negligible for the ND protocol execution time scale. For example, during $100\mu s$, nodes moving at 100kmph traverse
$2.7mm$, which is below the accuracy of RF ranging systems (in the
order of centimeters~\cite{multispectral}). However, in general,
mobility can have security implications. To see why, consider the $\pcrtl$ protocol. If nodes move during the protocol execution, it is important when they
estimate their location. At the very least, $A$ should estimate its location once when it sends the challenge, and again when it receives the response; whereas the responding node $B$ should estimate its location when it sends the response. But even this might be insufficient under high mobility: If $A$ measures its location at the beginning of the message, while $B$ measures the ToF at the end of the message, there may be space for a stealthy relay attack. Introducing mobility and a dynamically changing NLOS delay in our model is an interesting direction of our future work.

\textbf{Medium Access Control and Jamming.}
For simplicity, we do not introduce any MAC restrictions into the model. Hence,
a node is able to simultaneously receive any finite number of messages, even though in reality it is limited )to one message, or more for CDMA-like technologies).
We could introduce additional rules that model radio interference, e.g.,
set links \emph{down} if two (or more, depending on the node transceiver capabilities) simultaneous transmissions take place. However, this would \emph{not} affect any of our results. Notably, the availability properties require links to be \emph{up}, but they are agnostic as to why links are \emph{up} or \emph{down}. Similarly, jamming would not affect our results either: we capture jamming with links being \emph{down}, thus availability implies, among other things, no jamming.

\textbf{Inaccuracies.}
We assume correct nodes have accurate time and location information.
However, in reality, inaccuracies are possible. Regarding time, clocks may be coarse-grained, they can drift, especially if the synchronization protocol fails, or the node may encounter difficulties in estimating message reception times over a noisy channel. Regarding location, infrastructure (e.g., Global Positioning System (GPS), or base stations) providing location information may be temporarily unavailable, or localization algorithms may be coarse grained. Some of the inaccuracies can be decreased: For example, averaging ToF over many messages decreases estimation errors. But some inaccuracy in time and location is unavoidable.

As secure ND protocols rely on distance estimates, their effectiveness can be affected by such inaccuracies. For T-protocols, and even more so for TL-protocols, inaccuracies hinder availability: they can lead to ToF estimates seemingly above the threshold for T-protocols, and make the two distance estimates diverge for
TL-protocols. The only way to cope with these is to introduce some tolerance
margins for measurements. Nonetheless, this would affect correctness: The higher the tolerance margin, the more space is left for fast relay attacks. This manifests the unsurprising tension between correctness and availability. Introducing inaccuracies explicitly into the framework is an interesting component for future work.

\textbf{Physical Layer Attacks.}
The messages considered in our framework, albeit at the physical layer, are
composed of ``atomic'' components, such as nonces and identifiers, typically
assumed in formal security frameworks. In~\cite{clulow06sonear}, Clulow et al.
pointed out a number of physical layer attacks against DB protocols, working at the symbol (or bit) level. In the case of \emph{external} adversaries, as considered in our ND specification, the attacks proposed in~\cite{clulow06sonear} can result in a (perceivably) negative $\dr$. This can still be expressed in our model, hence our framework (notably the ``atomicity'' assumptions) is not limited with respect to those attacks. However, this is not the case for \emph{internal} adversaries, which we discuss in the \emph{Open Problems} section below.

%Furthermore, it might be possible that there exist physical layer
%attacks that would render our framework unfeasible.

\subsection{Protocol Comparison}\label{sec:comparison}

\textbf{T-protocols versus TL-protocols.}
TL-protocols are less restrictive than T-protocols in term of correctness: They do not need the notion of ND range, $\rng$, needed by T-protocols, and they are secure as long as $\dr > 0$ (always true, unless th above-discussed inaccuracies and attacks come into play), while T-protocols require the $\dr$ above $\rng\vel^{-1}$. In contrast, TL-protocols suffer in terms of availability: (i) they require location-aware nodes with secure location information, a far from trivial requirement, and (ii) they do not work for links with non-zero NLOS delay. We make a small note here on the nature of NLOS communication: Although there may be an obstacle between two nodes, it can still be possible to calculate the LOS message
arrival time.\footnotemark\ This, however, requires special care when
selecting/designing a wireless receiver. Another practical disadvantage of TL-protocols is their requirement that the signal propagation speed be $\vel = \vela$ (Note: it is reasonable to assume $\vela = c$, the
speed of light); this limits TL-protocols to RF and other electromagnetic wave
communications, while T-protocols can be used for lower speed technologies such as ultrasound.

\footnotetext{If the LOS communication path is blocked by an obstacle, the LOS
component of the received signal will be attenuated, and some NLOS components
might arrive at the receiver with higher power. However, if the earlier-arriving LOS component is not too weak, with enough care it can be possible to detect it, calculate message reception time and the resultant LOS propagation delay.}

%All the adversary models in this paper capture the technically feasible yet
%non-trivial ability to send and receive messages at the same time. For a weaker
%security result, one could assume that an adversarial node must receive the
%whole message before it can relay it. For such an adversary, a protocol whose
%every messages duration is longer than $\frac{\rng}{\vel}$ would solve ND (by
%Theorem~\ref{theorem:tpl}).

\textbf{B-protocols versus CR-protocols.}
B-protocols are conceptually simpler and have less stringent requirements for availability, requiring that links be \emph{up} for shorter periods than those needed by CR-protocols. In contrast, B-protocols require tightly synchronized
clocks, thus being impractical for many applications. In terms of correct (secure) operation, CRT-protocols require $\dr$, the minimum relaying delaye, to be twice as large as that required by BT-protocols (for the same $\rng$).

%Finally, we note that the requirement for links to up for CR-protocols could
%be loosened: For example the link does not need to be up all the time in both
%directions. We chose not to dive into these details for the sake of clarity and
%brevity.

\subsection{Open Problems}\label{sec:openproblems}

We observe that it is impossible to prove the correctness of the original 1993 distance bounding (DB) protocol by Chaums and Brands~\cite{Brands93DB} either in our framework or in the framework by Meadows et al.~\cite{meadows06db} that deals with DB protocols. First, the Brands-Chaum protocol uses commitments and an XOR operation; although the XOR operation is modeled in~\cite{meadows06db}, it cannot be used as it is in the Brands-Chaum protocol. More important, the Brands-Chaum protocol includes a \emph{rapid-bit-exchange} (RBE) phase, during which nodes exchange single, fresh bits. This poses a problem for the usual modeling of freshness, that is, a message being fresh if it did not previously occur in a trace. Obviously, fresh RBE \emph{bits} will repeatedly occur in a trace, as more than two will be exchanged.

The situation becomes even more interesting if we consider internal
adversaries, that is, the execution of an ND (or DB) protocol with an adversarial node. In general, an attack is always possible: An adversarial node can collude with another adversarial node that is a neighbor
of (is closer to) the victim node, and have it execute the ND or DB protocol on its behalf \cite{Brands93DB, meadows06db}. However, with additional assumptions, for example, that ``there is only one adversary node'' \cite{Brands93DB} or that ``nodes are prohibited to share cryptographic keys'' \cite{bussard04thesis}), some security guarantees can be claimed.

Nonetheless, in the presence of internal adversaries, the
physical layer attacks in Clulow et al.~\cite{clulow06sonear} are
much more significant than in the presence of external adversaries. We believe these types of attacks should be represented in any framework to
prove the security of ND or DB protocols against internal adversaries. This would
require a shift from a model that considers messages to one that considers physical communication layer symbols. Interestingly, this resembles the requirement to  properly model the DB RBE. But this should not be a big surprise: RBE was introduced specifically to deal with internal attackers. The way to develop these models remains an open question.


==> intro.tex <==
\section{Introduction}

Wireless communication systems have been developed and deployed in increasing
numbers and for diverse technologies, enabling a broad spectrum of
applications. Nonetheless, although emerging wireless networking and mobile
computing technologies offer a new rich set of tools, they also open the door
to new vulnerabilities, primarily because wireless communication makes
eavesdropping and injection of messages easy. Realizing that attacks against a
wireless system can be perpetrated essentially anywhere and anytime, the
research community devised a large volume of solutions to secure wireless
networking protocols and applications.

Among these efforts, the problem of \emph{securing neighbor discovery} has
received significant attention. \emph{Neighbor discovery} (ND), that is,
discovering that a wireless device (node) is directly reachable without the
assistance of any other device, is a fundamental element for practically any
wireless system. As a result, an attack against ND, that is, misleading nodes
into believing they are neighbors when they are not, does not merely introduce
an artificial wireless communication link between the victim (misled) nodes.
%From the adversary's point of view, 
It is a simple method to
compromise and abuse the system functionality that builds on ND: It is
sufficient for the adversary to simply \emph{relay} messages from one point to
another in the network, and vice versa, without any message
modification, to stage what is often termed a
\emph{wormhole} attack.

The consequences of such attacks can vary and be devastating. Consider, for example, the neighbor discovery of an access point (AP) performed by a mobile host in a WiFi network that
allows access to networked resources. A relay attack may appear at first
benign, or even helpful, as it essentially extends the AP range. However, it
offers the adversary the opportunity to intercept and fully control
communications of mobile hosts that cannot reach the AP but are 'attracted' to
do so over the wormhole setup by the attacker. Similarly, for multi-hop
wireless communication: In a wireless sensor network, nodes are likely to send
their measurements to the sink over a path that includes a wormhole. In a
different setting, a relay attack can be the most effective pick-pocket or
lock-picking mechanism: The adversary approaches a victim user, carrying a
radio frequency identification (RFID) tag for payments or for opening a car,
garage, or office building door, she then relays communication between the RFID
tag reader and the victim's tag, when the user is far from the RFID reader, and
she gets a money charge through or physically accesses the building.

The basic approach against such relay attacks has been to protect the pair-wise
execution of ND protocols with the help of various forms of
\emph{distance bounding} (DB) \cite{Brands93DB,hu01packet,eriksson06truelink}:
A node estimates its distance to another node by measuring the signal
\emph{time-of-flight (ToF)} to and/or from that node; if and only if the
estimate is below a threshold, it declares it a neighbor. In spite of numerous
schemes that are built on this approach, surveyed in Sec.~\ref{sec:related},
there has been no proof that secure ND is indeed achieved. This gap was brought forth very recently. \cite{commag08}
first argued informally that the existing proposals left the problem largely
open and pointed out a common misconception in the notion of ND. Then,
\cite{asiaccs08} established that, indeed, even for the most basic form of ND, what
we term \emph{two-party ND}, it is \emph{impossible} for a large class of
protocols that rely on time measurements to secure ND.

More important than the impossibility result per se, this highlights the need
to prove the properties of security protocols. Developments over many years are
not a substitute for rigorous reasoning on the protocol properties. In fact, a
false feeling of trustworthy technology can lead to the deployment of solutions
(algorithms, protocols) that were never proven secure. The subsequent
discovery of attacks exploiting core design flaws rather than implementation
glitches could only be a natural aftermath. The second important message that
one can extract from \cite{asiaccs08} is the need to carefully take into
consideration the idiosyncracies of the particular environment of the system to
be secured. The basic observation behind the impossibility result is otherwise
seemingly straightforward: Obstacles or interference can prevent nearby nodes
from communicating directly, thus allowing the attacker to remain undetected
while misleading two near-by nodes into believing they are neighbors (when they
are not, precisely because of such obstructions).

An impossibility result, although it provides important insight into the
problem at hand, does not provide solutions. Another crucial question is
\emph{proving the security of specific ND protocols} (under assumptions lifting
the impossibility result, obviously). We make a first step in this direction in~\cite{asiaccs08}, proving correctness of a simple ND protocol. In this
paper, we continue on this path.
We refine and extend the framework of \cite{asiaccs08} (Sec.~\ref{sec:sys-model}), providing a precise mathematical model of a wireless network and the adversary. These refinements and extensions bring our framework closer to the real world, in terms of reasoning on protocol correctness, and enable us to define the more elaborate \emph{challenge-response (CR)} ND protocols we introduce in this paper (Sec.~\ref{sec:protocols}). We revisit one of the \emph{beacon (B)}
protocols considered in \cite{asiaccs08}, and investigate additional protocols in our technical report \cite{techrep}.
Furthermore, we propose \emph{more practical availability properties} (Sec.~\ref{sec:properties}) than those geared towards and sufficient for the quest for the impossibility result. Clearly, a secure ND protocol concluding its execution correctly only 'once in a lifetime' satisfies the specification in  \cite{asiaccs08} but it is not practical. In terms of further approaching practical instantiations, we also consider composability: We aim at results which hold when the secure ND protocols are used along with other protocols. All these elements lead to a precise problem specification, thus enabling us to develop proofs for secure ND protocols (Sec.~\ref{sec:proofs}). Before we conclude, we provide a discussion on the framework and the analysis performed in this paper, identify open problems (Sec.~\ref{sec:discussion}), and survey related work (Sec.~\ref{sec:related}).


==> related.tex <==
\section{Related Work}\label{sec:related}

The prevalent wormhole prevention mechanism is based on \emph{distance
bounding} (DB), which was first proposed by Brands and Chaum in
\cite{Brands93DB} to thwart a relay attack between two correct nodes, also
termed a \emph{mafia fraud}. Essentially, DB estimates the distance between two
nodes, with the guarantee that it is not smaller from their real distance.
Subsequent proposals contributed in aspects such as mutual authentication
\cite{capkun03sector}, efficiency \cite{hancke05RFIDDB}, operation in noisy
environments \cite{munilla06dbvoid, singelee07dbnoisy}, and resistance to
execution of the protocol with a colluding group of adversarial nodes
\cite{bussard04thesis,reid06relayattacks}. In the latter, the attack termed
\emph{terrorist fraud} is thwarted under the assumption that adversarial nodes
do not expose their private cryptographic material; if not, one adversarial
node can undetectably impersonate another and successfully stage a terrorist
fraud. \emph{Authenticated ranging}, proposed by \v{C}apkun and Hubaux in
\cite{capkun06securepos}, lifts the technically non-trivial requirement of
rapid response (present in all the above protocols), at the expense of not
being resilient to a \emph{distance fraud}, when the protocol is executed with
a \emph{single, non-colluding} adversarial node \cite{bussard04thesis}.
Finally, two other ND protocols that rely only on time measurements are the
temporal packet leashes \cite{hu01packet} (recall the $\pbt$ is essentially a
temporal packet leash) and TrueLink \cite{eriksson06truelink} (neither
resistent to the distance fraud). The authors of~\cite{hu01packet} also
proposed geographical packet leashes, which rely on nodes being location-aware. This protocol is quite similar to the TL-protocol introduced in~\cite{asiaccs08}. But
we emphasize the difference: the latter protocol requires clock synchronization
as tight as that for temporal packet leashes, making it essentially a
combination of temporal and geographical leashes, thus achieving secure ND in
an environment with obstacles.

A number of other secure ND schemes is proposed in the literature. Most of them
rely on other wireless nodes or infrastructure, which may be (sometimes)
unavailable, e.g., in  WLAN or RFID systems. The approach of Poovendran and
Lazos \cite{poovendran07graphwormholes} relies on trusted, location-aware nodes
(\emph{guards}) to bootstrap ND. Hu and Evans have proposed a ND scheme
utilizing properties of directional antennas in
\cite{HuEvans04DirectionalAntennas}. In
\cite{maheshwairi07wormholeconnectivity}, Maheshwairi et al. propose to use
$k$-hop connectivity information obtained with a non-secure ND mechanism, and
to inspect it for \emph{forbidden structures}. Buttyan et al. also propose to
use statistic of the connectivity graph, leading to a centralized framework,
in~\cite{ButtyanDV05}. Another centralized approach by Wang et al.
\cite{WangBhargava04WormholeVisualization} uses approximate distance
measurements to visualize the network and enable a human operator to detect a
wormhole attack. Finally, Rasmussen and \v{C}apkun propose to use RF
fingerprinting for secure ND~\cite{rasmussen06RFF}. Although this is a
promising approach, it needs more practical investigation, notably about the
feasibility of RF fingerprint forging.

% MIGHT WANT TO BRING BACK, IF ROOM:
%The wormhole attack, in its symptoms, bears similarity to two other fundamental
%and hard to detect attacks. On one hand, a wormhole end can be perceived as a
%\emph{Sybil} node, with messages tied to different identities being transmitted
%by a single node. Hence, seemingly, a Sybil node detection mechanism
%\cite{newsome04sybil} could be used to thwart relay attacks. However, a
%wormhole can selectively relay the messages of a single node, and still be
%effective (e.g. Figure~\ref{fig:proof}, setting $\set^c$). On the other hand,
%as in the \emph{node replication} attack, messages tied to a single identity
%are transmitted by more than one node. However, node replication is harder to
%detect than a wormhole attack: schemes that address node replication
%\cite{parno05replication,conti07replication} focus on probabilistically
%detecting replicas located in remote parts of the network and require that
%nodes are location-aware. Obviously, a long-range wormhole can be easily (and
%deterministically) prevented using geographical packet leashes.

%%REVIVED FROM
The relay attack has been investigated in some recent works. One example is
\cite{hancke06relayattacks}, where Hancke demonstrates a relay attack using
only off-the-shelf hardware components, with a delay of around $20\mu s$.
In~\cite{reid06relayattacks} Reid et al. discuss using more sophisticated
microwave repeaters to achieve nanosecond level relaying delays. We also refer
an interested reader to a more theoretical work on relay (and other) physical
layer attacks on DB by Clulow et al.~\cite{clulow06sonear}, with a practical
follow-up in \cite{hancke08attackondb}, implementing some of these attacks
against two commercial radio receivers used in RFID and sensor networks.

Recently, there has been a rising interest in formalizing analysis of security
protocols in wireless networks. We mention works focusing on the security of
routing~\cite{nanz06framework, acs06provsecODrouting, papadimitratos06routing,
YangBaras03routing}, local area networking~\cite{he05proof80211}, or broadcast
authentication~\cite{hanna08sledge}. Closer to our work, the problem of DB has
been treated formally in~\cite{meadows06db} by Meadows et al. Their paper is
concerned with distance estimation rather than ND, but more importantly, the
approach is different. The authors of~\cite{meadows06db} build on top of
existing formal approaches~\cite{cervesato05authlogic, PavlovicD:ESORICS06}
tailored for ``classical'' security protocols, and augments it with a notion of
distance based on time-stamps. However, it is not clear how neighborhood would
be defined in this framework, nor how to model a protocol that uses location
information, such as $\pcrtl$. Beyond this, an interesting characteristic of their
approach is that there is no explicit notion of an adversary. On the contrary,
our approach starts with an explicit model of a wireless environment, including
node location, state of wireless links, and an explicit adversary, controlling
a number of nodes in the network. A potential advantage of this, although not
shown in this paper, is that attack scenarios can be expressed in our model,
whereas in~\cite{meadows06db} a collusion attack is described in an
informal manner.

